LLM-Driven Kernel Evolution: Automating Driver Updates in Linux

Linux kernel evolution breaks drivers through API/ABI changes, semantic shifts, and security-hardening updates. We introduce DRIVEBENCH, an executable corpus of kernel$\rightarrow$driver co-evolution cases, and AUTODRIVER, a closed-loop, LLM-driven system for automating driver maintenance. The system integrates prompt engineering, multi-agent collaboration, static analysis, and iterative validation to ensure that generated patches are not only syntactically correct but also functionally and semantically consistent with kernel conventions. The corpus spans v5.10-v6.10 with 235 validated cases drawn from 612 candidates. In evaluation across 55 cases, AUTODRIVER achieves 56.4% compilation success; QEMU-based boot verification indicates that compiled patches preserve driver initialization in most instances. By releasing DRIVEBENCH and tooling, we enable reproducible research and a practical route to continuous, safe co-evolution of drivers with the Linux kernel.

==> content/tables/batch.tex <==
\begin{table*}[t]
  \centering
  \small
  \setlength{\tabcolsep}{6pt}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{
    >{\raggedright\arraybackslash}p{0.20\linewidth}
    >{\centering\arraybackslash}p{0.10\linewidth}
    >{\centering\arraybackslash}p{0.15\linewidth}
    >{\centering\arraybackslash}p{0.15\linewidth}
    >{\centering\arraybackslash}p{0.15\linewidth}
    >{\centering\arraybackslash}p{0.15\linewidth}
  }
    \toprule
    \textbf{Issue Type} &
    \cellcolor{orange!10}\textbf{Total} &
    \cellcolor{green!10}\textbf{DS Gen\&Apply} &
    \cellcolor{green!10}\textbf{DS Compile} &
    \cellcolor{blue!10}\textbf{GPT Gen\&Apply} &
    \cellcolor{blue!10}\textbf{GPT Compile} \\
    \midrule

    \rowcolor{catrow}
    \multicolumn{6}{l}{\textit{Automated Patch Validation Results}}\\
    \addlinespace[2pt]

    Optimisation & 50 & 49 & 16 & 50 & 9 \\
    Deprecation  & 36 & 36 & 23 & 36 & 10 \\
    Removal      & 16 & 16 & 6  & 16 & 3 \\
    Rename       & 3  & 3  & 2  & 3  & 1 \\
    Regression   & 8  & 7  & 3  & 8  & 2 \\
    \midrule
    \textbf{Total/Average} & \textbf{113} & \textbf{111} & \textbf{50} & \textbf{113} & \textbf{25} \\
    \bottomrule
  \end{tabular}
  \caption{
    \emph{Batch test results across five issue types.}
    DeepSeek-Coder (DS) consistently achieves higher compilation reliability than GPT-4o.
    Values denote successful cases out of total attempts.
  }
  \label{tab:batch-results}
\end{table*}

==> content/tables/metrics.tex <==
\begin{table*}[t]
  \centering
  \small
  \setlength{\tabcolsep}{6pt}
  \begin{tabular}{
    >{\raggedright\arraybackslash}p{0.15\linewidth}
    >{\raggedright\arraybackslash}p{0.30\linewidth}
    >{\raggedright\arraybackslash}p{0.30\linewidth}
    >{\raggedright\arraybackslash}p{0.15\linewidth}
  }
    \toprule
    \textbf{Layer} &
    \cellcolor{orange!10}\textbf{Objective} &
    \cellcolor{green!10}\textbf{Implementation / Tool} &
    \cellcolor{gray!08}\textbf{Granularity} \\
    \midrule

    \rowcolor{catrow}
    \multicolumn{4}{l}{\textit{Syntactic and Structural Validation}}\\
    \addlinespace[1pt]

    Structural &
    Validate diff format, context, and path integrity. &
    \texttt{git apply --check}, diff-tree analysis. &
    File / Hunk. \\
    \addlinespace[2pt]

    Syntactic &
    Ensure grammatical correctness of C code. &
    Parser frontend (\texttt{libclang}). &
    Function / AST node. \\
    \midrule

    \rowcolor{catrow}
    \multicolumn{4}{l}{\textit{Semantic and Behavioural Evaluation}}\\
    \addlinespace[1pt]

    Semantic &
    Measure equivalence of AST edit operations. &
    $\mathrm{ASTSim}$ (Eq.~\ref{eq:astsim}). &
    Function / Patch. \\
    \addlinespace[2pt]

    Style \& Convention &
    Check coding-standard compliance. &
    \texttt{checkpatch.pl}, \texttt{clang-format}. &
    File / Patch. \\
    \addlinespace[2pt]

    Behavioural &
    Validate functional correctness via tests. &
    Subsystem-specific regression tests. &
    System / Submodule. \\
    \midrule

    \rowcolor{catrow}
    \multicolumn{4}{l}{\textit{Aggregated Assessment}}\\
    \addlinespace[1pt]

    Aggregated Score &
    Combine heterogeneous similarity signals. &
    Weighted static analysis (Eq.~\ref{eq:composite}). &
    Patch-level aggregate. \\
    \bottomrule
  \end{tabular}
  \caption{
    \emph{Summary of evaluation metrics.}
    Each layer captures distinct aspects of patch fidelity,
    progressing from syntactic validity to semantic and behavioural equivalence.
  }
  \label{tab:metric-summary}
\end{table*}

==> content/tables/results.tex <==
\begin{table*}[t!]
\caption{
Comprehensive evaluation on \benchmark{} for \textit{LLM-Driven Kernel Evolution}.
\textbf{Dark gray} marks best overall, \textbf{light gray} best among open-source models.
Green cells indicate top-3 ranks within each group.
\textbf{Avg.} denotes the average over all layers in the \textit{Patch Evaluation Suite}
(\textit{Structural}, \textit{Syntactic}, \textit{Semantic}, \textit{Style}, \textit{Behavioural}, \textit{Aggregated}).
}
\label{tab:kernelevolutionresults}
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{rr|c|c|cccccc|cccccc}
 & & & &
\rotatebox{60}{Patch Accuracy} &
\rotatebox{60}{Build Success} &
\rotatebox{60}{Tool Usage Rate} &
\rotatebox{60}{Inference Stability} &
\rotatebox{60}{Patch Correctness} &
\rotatebox{60}{Test Pass Rate} &
\rotatebox{60}{Structural Validity} &
\rotatebox{60}{Syntactic Correctness} &
\rotatebox{60}{AST Equivalence} &
\rotatebox{60}{Convention Compliance} &
\rotatebox{60}{Behavioural Fidelity} &
\rotatebox{60}{Composite Fidelity Score} \\
\multicolumn{2}{r|}{\textbf{Methods}} & \textbf{Rank} & \textbf{Avg.} &
\multicolumn{6}{r|}{\cellcolor{orange!10}\textbf{Numerical / Binary Metrics}} &
\multicolumn{6}{r}{\cellcolor{yellow!10}\textbf{Multi-Layer Patch Evaluation Suite}} \\
\midrule

\rowcolor{catrow}
\multicolumn{16}{l}{\textit{Baselines (Non-LLM)}} \\
Coccinelle & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
clang static analyzer & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
LinuxDiff (heuristic) & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule

\rowcolor{catrow}
\multicolumn{16}{l}{\textit{Rule-based / Statistical Models}} \\
Code2Vec & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
DeepPatch (2019) & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
PatchNet (2020) & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule

\rowcolor{catrow}
\multicolumn{16}{l}{\textit{One-Shot / No-Tooling LLMs}} \\
GPT-4o-mini & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
GPT-4o & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Claude 3.5 Sonnet & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Claude Haiku & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Gemini 2.0 Flash & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
DeepSeek R1 & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule

\rowcolor{catrow}
\multicolumn{16}{l}{\textit{Proprietary Models (API)}} \\
GPT-5 (API) & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Claude 3.5 Sonnet (API) & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Gemini 2.0 Pro & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
DeepSeek Coder R1 (API) & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Mistral Codestral 22B (API) & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
XAI Grok 4 & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Amazon Olympus & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule

\rowcolor{catrow}
\multicolumn{16}{l}{\textit{Open-Source Models}} \\
Llama 3.1 8B Instruct & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Llama 3.1 70B Instruct & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Qwen 2.5 14B & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Qwen 2.5 32B & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
StarCoder2 15B & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
CodeLlama 34B & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
DeepSeek Coder 33B & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Mistral Codestral 22B & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Phi-3-medium & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Yi-1.6 9B & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Zephyr 7B-beta & & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}%
}
\end{table*}
